On the Spectrum and Spacetime Supersymmetry of Heterotic Ambitwistor String

We analyse the BRST cohomology of the Ramond sector of heterotic ambitwistor theory. We also write the free string field theory action and compute the supersymmetry transformations.

==> packages.tex <==
\usepackage[a4paper, margin=2cm]{geometry}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{hyperref}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{amsbsy}
\usepackage{bm}
\usepackage{mathrsfs}
\usepackage{slashed}
\usepackage{graphicx}
%\usepackage{tikz-cd}
\usepackage{fancyhdr}

\newcommand{\db}{\bar{\partial}}
\newcommand{\pd}{\partial}
\newcommand{\al}{\alpha}
\newcommand{\bt}{\beta}
\newcommand{\ad}{\dot{\alpha} }
\newcommand{\bd}{\dot{\beta}}
\newcommand{\bra}{\langle}
\newcommand{\ket}{\rangle}
\newcommand{\bx}{\square}
\newcommand{\tc}{\tilde{c}}
\newcommand{\tb}{\tilde{b}}
\newcommand{\fa}{\frac{\alpha'}{4} }
\newcommand{\mr}{\mathbin{\color{red}-}}
\newcommand{\pr}{\mathbin{\color{red}+}}

\numberwithin{equation}{section}

\newtheoremstyle{henrique}      %Name
  { }                                              % Space above
  {}                                              % Space below
  {\normalfont}                            % Body font
  {}                                              % Indent amount
  {\bfseries}                                % Theorem head font
  {.}                                             % Punctuation after theorem head
  { }                                             % Space after theorem head, ' ', or \newline
  {}                                              % Theorem head spec (can be left empty, meaning `normal')
\theoremstyle{henrique}
\newtheorem{teo}{Theorem}[section]
\newtheorem{defi}{Definition}[section]
\newtheorem{lema}{Lemma}[section]
\newtheorem{corol}{Corollary}[section]
\newtheorem{prop}{Proposition}[section]

\hypersetup{colorlinks=false, urlbordercolor={1 0 0}, linkbordercolor={0 0 1}, citebordercolor={0 0 1}}

